Retrospective Cost-based Extremum Seeking Control with Vanishing Perturbation for Online Output Minimization

Extremum seeking control (ESC) constitutes a powerful technique for online optimization with theoretical guarantees for convergence to the neighborhood of the optimizer under well-understood conditions. However, ESC requires a nonconstant perturbation signal to provide persistent excitation to the target system to yield convergent results, which usually results in steady state oscillations. While certain techniques have been proposed to eliminate perturbations once the neighborhood of the minimizer is reached, system modifications and environmental perturbations can suddenly change the minimizer and nonconstant perturbations would once more be required to convergence to the new minimizer. Hence, this paper develops a retrospective cost-based ESC(RC/ESC) technique for online output minimization with a vanishing perturbation, that is, a perturbation that becomes zero as time increases independently from the state of the controller or the controlled system. The performance of the proposed algorithm is illustrated via numerical examples.

==> PackagesCommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% PACKAGES %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{amsfonts}
% \usepackage{amsthm}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}[section]
% \theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
% \newtheorem{def_chap}{Definition}[chapter]
% % \newtheorem{definitionSec}{Definition}[subsection]
\newtheorem{exmp}{Example}[section]
% \newtheorem{exmp_chap}{Example}[chapter]
% \newtheorem{exmpSec}{Example}[subsection]
\newtheorem{fact}{Fact}[section]
% \newtheorem{fact_chap}{Fact}[chapter]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{factSec}{Fact}[subsection]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{problem}{Problem}[section]
% \newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}[section]

\newtheorem{prob}{Problem}[section]

\usepackage{graphicx}
% \usepackage{epsfig}
\usepackage{epstopdf}
% \usepackage{math tools}
% \usepackage{color}
% \usepackage[utf8]{inputenc}
%\pagestyle{plain}

% \usepackage{subfigure}
% \usepackage{subfig}
\usepackage{float} 
\usepackage[skip=0pt,font=footnotesize]{caption}
% \usepackage{wrapfig}%   wrap figures/tables in text (i.e., Di Vinci style)
% \usepackage[export]{adjustbox}

% \usepackage{geometry}
% \usepackage{indentfirst}


% \usepackage{epsfig} % for postscript graphics files

% \usepackage{lastpage}
% \usepackage{fancyhdr}
% \pagestyle{fancy} 
% \cfoot{\thepage\ of \pageref{LastPage}}
% \fancyhead{}
% \renewcommand{\headrulewidth}{0pt}

% \usepackage{mathptmx} % assumes new font selection scheme installed
% \usepackage{times} % assumes new font selection scheme installed


% \usepackage[mathscr]{euscript}

% \usepackage{newtxtext}
% \usepackage{newtxmath}

% \usepackage{subfiles}
% \usepackage{cancel}
% \usepackage{imakeidx}

%\usepackage{citesort}
%\usepackage[fleqn]{amsmath}
%\usepackage{fullpage}
%\usepackage[top=0.75in,bottom= 0.75in,left = 0.75in, right = 0.75in]{geometry}
\usepackage[margin = 1in]{geometry}

%\parskip = -0.5pt
%\parindent = 2pt %0in


%\usepackage{multicol}
%\usepackage{caption}
%\usepackage[skip=2pt]{caption}
%\usepackage[skip=1pt,font=footnotesize]{caption}
%\usepackage[skip=1pt,font=small]{caption}
\usepackage{subcaption}


\usepackage{etaremune}



% \usepackage{tikz}
% \usetikzlibrary{shapes,arrows,calc,positioning}
% \tikzstyle{bigblock} = [draw, fill=blue!20, rectangle, 
%     minimum height=6em, minimum width=8em]
% \tikzstyle{medblock} = [draw, fill=blue!20, rectangle, 
%     minimum height=4em, minimum width=4em]    
% \tikzstyle{mux} = [draw, fill=black!20, rectangle, 
%     minimum height=5em, minimum width=0.1em]    
% \tikzstyle{smallblock} = [draw, fill=blue!20, rectangle, 
%     minimum height=2em, minimum width=3em]
    
% \tikzstyle{data_block} = [draw, fill=green!20, rectangle, 
%     minimum height=2em, minimum width=3em]
% \tikzstyle{ops_block} = [draw, fill=blue!20, rectangle, 
%     minimum height=2em, minimum width=3em]    
% \tikzstyle{est_block} = [draw, fill=red!20, rectangle, 
%     minimum height=2em, minimum width=3em]    
    
% \tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm,minimum height=0.5cm]
% \tikzstyle{signal} = [coordinate]
% \tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
% \tikzstyle{block} = [draw, fill=blue!20, rectangle, 
%     minimum height=3em, minimum width=9em]
% \tikzstyle{blockS} = [draw, fill=blue!20, rectangle, 
%     minimum height=3em, minimum width=4em]    
% \tikzstyle{input} = [coordinate]
% \tikzstyle{output} = [coordinate]
% \usetikzlibrary{matrix}

% \usetikzlibrary{positioning}
% \usetikzlibrary{math} 


\input{TikzStuff}

\usepackage{hyperref}
\usepackage{xcolor}
\hypersetup{
    colorlinks,
    linkcolor={blue!100!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}

% \usepackage{diagbox}


%\newtheorem{definition}{Definition}[section]
%\usepackage{biblatex}
% \addbibresource{mendeley_v2.bib}

% \usepackage[square, numbers, sort&compress]{natbib} 
% \setcitestyle{square braces, numbers}
%\usepackage{cite}



%\usepackage[nomarkers,figuresonly]{endfloat}

% \renewcommand{\familydefault}{\rmdefault}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% COMMANDS %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\nn}{\nonumber}
\newcommand{\matl}{\left[ \begin{array}}
\newcommand{\matr}{\end{array} \right]}
\newcommand{\matls}{\left[ \begin{smallmatrix}}
\newcommand{\matrs}{\end{smallmatrix} \right]}
\newcommand{\isdef}{\stackrel{\triangle}{=}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\inv}{^{-1}}
\newcommand{\row}[1]{{\rm row}_{#1}}
\newcommand{\col}[1]{{\rm col}_{#1}}
\newcommand{\arrowup}[1]{\stackrel{#1}{\SLeftarrow}}
\newcommand{\smin}{\stackrel{\min}{\sim}}
\newcommand{\jw}{\jmath \omega}
\newcommand{\omegan}{\omega_{\rm n}}
\newcommand{\omegad}{\omega_{\rm d}}
\newcommand{\omegar}{\omega_{\rm r}}
\newcommand{\omegani}{\omega_{{\rm n}i}}
\newcommand{\omegans}[1]{\omega_{{\rm n}_{#1}}}
\newcommand{\MSig}{{\mit\Sigma}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\vect}[1]{\overset{\rightharpoonup}{#1}}
\newcommand{\HS}{\hat S}
\newcommand{\HI}{\hat I}
\newcommand{\rmThat}{{\hat{\rm T}}}
\newcommand{\asthat}{{\hat*}}
\newcommand{\dpder}[2]{\displaystyle\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\der}[2]{\mbox{$\frac{d{#1}}{d{#2}}$}}
\newcommand{\dder}[2]{\displaystyle{\frac{d{#1}}{d{#2}}}}
\newcommand{\pder}[2]{\mbox{$\frac{\partial {#1}}{\partial {#2}}$}}
\newcommand{\dt}{{\rm d}t}
\newcommand{\dx}{{\rm d}x}
\newcommand{\p}{\partial}
\newcommand{\pt}{\partial_t}
\newcommand{\ptt}{\partial^2_t}
\newcommand{\px}{\partial_x}
\newcommand{\pxx}{\partial^2_x}
\newcommand{\pp}{\partial{^2}}
\newcommand{\tr}{{\rm tr}\,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%\DeclareMathOperator{\tr}{tr}
\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}
\newcommand{\rma}{{\rm a}}
\newcommand{\rmb}{{\rm b}}
\newcommand{\rmc}{{\rm c}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\rme}{{\rm e}}
\newcommand{\rmf}{{\rm f}}
\newcommand{\rmg}{{\rm g}}
\newcommand{\rmh}{{\rm h}}
\newcommand{\rmi}{{\rm i}}
\newcommand{\rmj}{{\rm j}}
\newcommand{\rmk}{{\rm k}}
\newcommand{\rml}{{\rm l}}
\newcommand{\rmm}{{\rm m}}
\newcommand{\rmn}{{\rm n}}
\newcommand{\rmo}{{\rm o}}
\newcommand{\rmp}{{\rm p}}
\newcommand{\rmq}{{\rm q}}
\newcommand{\rmr}{{\rm r}}
\newcommand{\rms}{{\rm s}}
\newcommand{\rmt}{{\rm t}}
\newcommand{\rmu}{{\rm u}}
\newcommand{\rmv}{{\rm v}}
\newcommand{\rmw}{{\rm w}}
\newcommand{\rmx}{{\rm x}}
\newcommand{\rmy}{{\rm y}}
\newcommand{\rmz}{{\rm z}}
\newcommand{\BBA}{{\mathbb A}}
\newcommand{\BBB}{{\mathbb B}}
\newcommand{\BBC}{{\mathbb C}}
\newcommand{\BBD}{{\mathbb D}}
\newcommand{\BBE}{{\mathbb E}}
\newcommand{\BBF}{{\mathbb F}}
\newcommand{\BBG}{{\mathbb G}}
\newcommand{\BBH}{{\mathbb H}}
\newcommand{\BBI}{{\mathbb I}}
\newcommand{\BBJ}{{\mathbb J}}
\newcommand{\BBK}{{\mathbb K}}
\newcommand{\BBL}{{\mathbb L}}
\newcommand{\BBM}{{\mathbb M}}
\newcommand{\BBN}{{\mathbb N}}
\newcommand{\BBO}{{\mathbb O}}
\newcommand{\BBP}{{\mathbb P}}
\newcommand{\BBQ}{{\mathbb Q}}
\newcommand{\BBR}{{\mathbb R}}
\newcommand{\BBS}{{\mathbb S}}
\newcommand{\BBT}{{\mathbb T}}
\newcommand{\BBU}{{\mathbb U}}
\newcommand{\BBV}{{\mathbb V}}
\newcommand{\BBW}{{\mathbb W}}
\newcommand{\BBX}{{\mathbb X}}
\newcommand{\BBY}{{\mathbb Y}}
\newcommand{\BBZ}{{\mathbb Z}}

\newcommand{\real}{{\mathbb{R}}}
\newcommand{\comp}{{\mathbb{C}}}
\newcommand{\realR}{\mathbb{R}}

\newcommand{\SA}{{\mathcal A}}
\newcommand{\SB}{{\mathcal B}}
\newcommand{\SC}{{\mathcal C}}
\newcommand{\SD}{{\mathcal D}}
\newcommand{\SE}{{\mathcal E}}
\newcommand{\SF}{{\mathcal F}}
\newcommand{\SG}{{\mathcal G}}
\newcommand{\SH}{{\mathcal H}}
\newcommand{\SI}{{\mathcal I}}
\newcommand{\SJ}{{\mathcal J}}
\newcommand{\SK}{{\mathcal K}}
\newcommand{\SL}{{\mathcal L}}
\newcommand{\SM}{{\mathcal M}}
\newcommand{\SN}{{\mathcal N}}
\newcommand{\SO}{{\mathcal O}}
\newcommand{\SP}{{\mathcal P}}
\newcommand{\SQ}{{\mathcal Q}}
\newcommand{\SR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\ST}{{\mathcal T}}
\newcommand{\SU}{{\mathcal U}}
\newcommand{\SV}{{\mathcal V}}
\newcommand{\SW}{{\mathcal W}}
\newcommand{\SX}{{\mathcal X}}
\newcommand{\SY}{{\mathcal Y}}
\newcommand{\SZ}{{\mathcal Z}}
\newcommand{\BFA}{{\bf A}}
\newcommand{\BFB}{{\bf B}}
\newcommand{\BFC}{{\bf C}}
\newcommand{\BFD}{{\bf D}}
\newcommand{\BFE}{{\bf E}}
\newcommand{\BFF}{{\bf F}}
\newcommand{\BFG}{{\bf G}}
\newcommand{\BFH}{{\bf H}}
\newcommand{\BFI}{{\bf I}}
\newcommand{\BFJ}{{\bf J}}
\newcommand{\BFK}{{\bf K}}
\newcommand{\BFL}{{\bf L}}
\newcommand{\BFM}{{\bf M}}
\newcommand{\BFN}{{\bf N}}
\newcommand{\BFO}{{\bf O}}
\newcommand{\BFP}{{\bf P}}
\newcommand{\BFQ}{{\bf Q}}
\newcommand{\BFR}{{\bf R}}
\newcommand{\BFS}{{\bf S}}
\newcommand{\BFT}{{\bf T}}
\newcommand{\BFU}{{\bf U}}
\newcommand{\BFV}{{\bf V}}
\newcommand{\BFW}{{\bf W}}
\newcommand{\BFX}{{\bf X}}
\newcommand{\BFY}{{\bf Y}}
\newcommand{\BFZ}{{\bf Z}}
\def\bbR{\mbox{\bbfnt R}}
\newcommand{\vspaceAnkit}{\vspace{-3pt}}
\newcommand{\shiftq}{{\textbf{\textrm{q}}}}

\newcommand{\ddt}{\dfrac{\rmd}{\rmd t}}
\newcommand{\ddx}{\dfrac{\rmd}{\rmd x}}






% \newtheoremstyle{factindented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{1.5em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}
% %\theoremstyle{factindented}


% \newtheoremstyle{indented}
%     {3pt}
%     {3pt}
%     {\addtolength{\leftskip}{3em}}
%     {}
%     {\bfseries}
%     {.}
%     {.5em}
%     {}

% \theoremstyle{indented}







% \newcommand{\SCA}{{\mathscr{A}}}
% \newcommand{\SCB}{{\mathscr{B}}}
% \newcommand{\SCU}{{\mathscr{U}}}

\newcommand{\Star}{^{*}}

%\newcommand{\scM}{{\mathscr M}}
\newcommand{\scM}{{\mathcal M}}

\newcommand{\neweqline}{\ensuremath{\nn \\ &\quad }}


\newcommand{\framedot}[2]{\stackrel{{\rm #1}\bullet}{#2}}
\newcommand{\frameddot}[2]{\stackrel{{\rm #1}\bullet \bullet}{#2}}

\newcommand{\polar}[1]{\ensuremath{r_{#1}e^{\jmath \theta_{#1}}}}

\renewcommand{\matl}{\begin{bmatrix}}
\renewcommand{\matr}{\end{bmatrix} }

\newcommand{\tarrow}[1]{\overset{\rightarrow}{#1}}

==> RCACStyle.tex <==



\newtheorem{theo}{Theorem}[section]
\newtheorem{prop}[theo]{Proposition}
\newtheorem{cor}[theo]{Corollary}
\newtheorem{defin}[theo]{Definition}
\newtheorem{fact}[theo]{Fact}
\newtheorem{lem}[theo]{Lemma}
\newtheorem{exam}[theo]{Example}

%\newtheorem*{proof}{Proof}
\newtheorem{prob}[theo]{Problem}

\newtheorem{assume}[theo]{Assumption}


% \renewcommand{\thefigure}{\arabic{chapter}.\arabic{section}.\arabic{figure}}
% \setcounter{figure}{1}


\newcommand{\trans}{^{\mbox{\scriptsize\sf T}}}


\renewcommand{\labelenumi}{\it\roman{enumi}\rm)}

\DeclareMathOperator{\co}{conv}

\DeclareMathOperator{\cone}{cone}

\DeclareMathOperator{\polar}{polar}

\DeclareMathOperator{\dcone}{d\mspace{-.5mu}cone}

\DeclareMathOperator{\coco}{coco}

\DeclareMathOperator{\Imag}{Im}

\DeclareMathOperator{\Real}{Re}

\DeclareMathOperator{\tr}{tr}

\DeclareMathOperator{\str}{str}  

\DeclareMathOperator{\rank}{rank}

\DeclareMathOperator{\defect}{def}

\DeclareMathOperator{\spann}{span}

\DeclareMathOperator{\aff}{affin}

\DeclareMathOperator{\ind}{ind}

\DeclareMathOperator{\spec}{spec}

\DeclareMathOperator{\mspec}{mspec}

\DeclareMathOperator{\roots}{roots}

\DeclareMathOperator{\mroots}{mroots}

\DeclareMathOperator{\diag}{diag}

\DeclareMathOperator{\revdiag}{revdiag}

\DeclareMathOperator{\Diag}{Diag}

\DeclareMathOperator{\volume}{volume}

\DeclareMathOperator{\area}{area}

\DeclareMathOperator{\Inert}{In}

\DeclareMathOperator{\vek}{vec}

\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator{\cl}{cl}

\DeclareMathOperator{\relcl}{relcl}

\DeclareMathOperator{\inter}{int}

\DeclareMathOperator{\relint}{relint}

\DeclareMathOperator{\bd}{bd}

\DeclareMathOperator{\relbd}{relbd}

\DeclareMathOperator{\fcone}{fcone}

\DeclareMathOperator{\ad}{ad}

\DeclareMathOperator{\sprad}{sprad}

\DeclareMathOperator{\spabs}{spabs}

\DeclareMathOperator{\nrad}{nrad}

\DeclareMathOperator{\reldeg}{reldeg}

\DeclareMathOperator{\sig}{sig}

\DeclareMathOperator{\card}{card}

\DeclareMathOperator{\glb}{glb}

\DeclareMathOperator{\lub}{lub}

\DeclareMathOperator{\essglb}{essglb}  

\DeclareMathOperator{\esslub}{esslub}

\DeclareMathOperator{\truth}{truth}

\DeclareMathOperator{\modd}{mod}

\DeclareMathOperator{\rem}{rem}

\DeclareMathOperator{\Arg}{arg}

%\DeclareMathOperator{\gcd}{gcd}

\DeclareMathOperator{\lcm}{lcm}

\DeclareMathOperator{\asin}{asin}

\DeclareMathOperator{\sech}{sech}

\DeclareMathOperator{\csch}{csch}

\DeclareMathOperator{\ecl}{ecl}

\DeclareMathOperator{\iso}{iso}

\DeclareMathOperator{\ebd}{ebd}

\DeclareMathOperator{\OLHP}{\rm OLHP}

\DeclareMathOperator{\CLHP}{\rm CLHP}

\DeclareMathOperator{\CRHP}{\rm CRHP}

\DeclareMathOperator{\ORHP}{\rm ORHP}

\DeclareMathOperator{\IA}{\rm IA}

\DeclareMathOperator{\OIUD}{\rm OIUD}

\DeclareMathOperator{\CIUD}{\rm CIUD}

\DeclareMathOperator{\COUD}{\rm COUD}

\DeclareMathOperator{\OOUD}{\rm OOUD}

\DeclareMathOperator{\UC}{\rm UC}




\renewcommand{\theenumi}{$\roman{enumi})$}
%\renewcommand{\theenumi}{\roman{enumi})}
\renewcommand{\labelenumi}{\theenumi}
%\setcounter{enumi}{2}--------to restart counter after last number


 
 
 
 
\newcommand{\0}{_{0}}
\newcommand{\subc}{_{\rm c}}


\newcommand{\vect}[1]{\overset{\rightharpoonup}{#1}}
\newcommand{\longarrow}{\hbox{$=$\hskip-.15em $\Rightarrow$}}
\def\tabrule{\noalign{\hrule}}

\newcommand{\tarrow}[1]{\overset{\rightarrow}{#1}}

%\newcommand{\tlrarrow}[1]{\overset{\leftrightarrow}{#1}}

\newcommand{\tlrarrow}[1]{\overset{\twoheadrightarrow}{#1}}%Use this if I want to distinguish multivectors---but why bother????????

%\newcommand{\tlrarrow}[1]{\overset{\rightarrow}{#1}}



\newcommand{\opendot}[1]{\stackrel{\circ}{#1}}
\newcommand{\soliddot}[1]{\stackrel{\bullet}{#1}}

\newcommand{\openddot}[1]{\stackrel{\circ\mspace{1mu}\circ}{#1}}
\newcommand{\solidddot}[1]{\stackrel{\bullet\mspace{1mu}\bullet}{#1}}
\newcommand{\mixeddot}[1]{\stackrel{\bullet\mspace{1mu}\circ}{#1}}



\newcommand{\framedotA}[1]{\stackrel{\rmA\bullet}{#1}}
\newcommand{\framedotB}[1]{\stackrel{\rmB\bullet}{#1}}
\newcommand{\framedotC}[1]{\stackrel{\rmC\bullet}{#1}}
\newcommand{\framedotD}[1]{\stackrel{\rmD\bullet}{#1}}
\newcommand{\framedotE}[1]{\stackrel{\rmE\bullet}{#1}}
\newcommand{\framedotI}[1]{\stackrel{\rmI\bullet}{#1}}
\newcommand{\framedotIprime}[1]{\stackrel{\rmI^\prime\bullet}{#1}}
\newcommand{\framedotAC}[1]{\stackrel{\rmA\rmC\bullet}{#1}}
\newcommand{\framedotS}[1]{\stackrel{\rmS\bullet}{#1}}
\newcommand{\framedotW}[1]{\stackrel{\rmW\bullet}{#1}}
\newcommand{\framedotM}[1]{\stackrel{\rmM\bullet}{#1}}

\newcommand{\framedotSC}[1]{\stackrel{\rmB\bullet}{#1}}
\newcommand{\framedotWHi}[1]{\stackrel{\rmW_i\bullet}{#1}}


\newcommand{\framedotBprime}[1]{\stackrel{\rmB\bullet'}{#1}}




\newcommand{\framedotalpha}[1]{\stackrel{\alpha\bullet}{#1}}

\newcommand{\framedotx}[1]{\stackrel{x\bullet}{#1}}
\newcommand{\framedoty}[1]{\stackrel{y\bullet}{#1}}
\newcommand{\framedotz}[1]{\stackrel{z\bullet}{#1}}


\newcommand{\framedotAalpha}[1]{\stackrel{\rmA\alpha\bullet}{#1}}
\newcommand{\frameddotAalpha}[1]{\stackrel{\rmA\alpha\bullet\bullet}{#1}}
\newcommand{\framedddotAalpha}[1]{\stackrel{\rmA\alpha\bullet\bullet\bullet}{#1}}

\newcommand{\framedotBalpha}[1]{\stackrel{\rmB\alpha\bullet}{#1}}

\newcommand{\framedots}[1]{\stackrel{\rmA s\bullet}{#1}}
\newcommand{\frameddots}[1]{\stackrel{\rmA s\bullet\bullet}{#1}}
\newcommand{\framedddots}[1]{\stackrel{\rmA s\bullet\bullet\bullet}{#1}}

\newcommand{\framedotK}[1]{\stackrel{\rmK\bullet}{#1}}

\newcommand{\framedotsi}[1]{\stackrel{\rmA s_i\bullet}{#1}}
\newcommand{\framedotsc}[1]{\stackrel{\rmA s_\rmc\bullet}{#1}}


\newcommand{\frameddotA}[1]{\stackrel{\rmA\bullet\bullet}{#1}}
\newcommand{\frameddotB}[1]{\stackrel{\rmB\bullet\bullet}{#1}}
\newcommand{\frameddotC}[1]{\stackrel{\rmC\bullet\bullet}{#1}}
\newcommand{\frameddotD}[1]{\stackrel{\rmD\bullet\bullet}{#1}}
\newcommand{\frameddotE}[1]{\stackrel{\rmE\bullet\bullet}{#1}}
\newcommand{\frameddotI}[1]{\stackrel{\rmI\bullet\bullet}{#1}}
\newcommand{\frameddotIprime}[1]{\stackrel{\rmI^\prime\bullet\bullet}{#1}}
\newcommand{\frameddotAC}[1]{\stackrel{\rmA\rmC\bullet\bullet}{#1}}
\newcommand{\frameddotS}[1]{\stackrel{\rmS\bullet\bullet}{#1}}
\newcommand{\frameddotW}[1]{\stackrel{\rmW\bullet\bullet}{#1}}
\newcommand{\frameddotM}[1]{\stackrel{\rmM\bullet\bullet}{#1}}
\newcommand{\framedotcyl}[1]{\stackrel{\rm cyl\bullet}{#1}}
\newcommand{\frameddotcyl}[1]{\stackrel{\rm cyl\bullet\bullet}{#1}}
\newcommand{\framedotsph}[1]{\stackrel{\rm sph\bullet}{#1}}
\newcommand{\frameddotsph}[1]{\stackrel{\rm sph\bullet\bullet}{#1}}

\newcommand{\framedotFSalpha}[1]{\stackrel{\rm FS\alpha\bullet}{#1}}

\newcommand{\framedotGHi}[1]{\stackrel{\rmG_i\bullet}{#1}}


 
\newcommand{\framedddotA}[1]{\stackrel{\rmA\bullet\bullet\bullet}{#1}}
\newcommand{\framedddotB}[1]{\stackrel{\rmB\bullet\bullet\bullet}{#1}}

\newcommand{\tp}[1]{{#1}^{\rm T}}
%\newcommand{\begin{align}}{\begin{align}}
%\newcommand{\ealign}{\end{align}}
\newcommand{\tpm}[1]{{#1}^{\rm -T}}
 
 
 
 
 
 
 
 
 
 
 
 

\newcommand{\modup}[1]{\stackrel{#1}{\equiv}}
\newcommand{\re}{\mbox{\rm Re}}
\newcommand{\im}{\mbox{\rm Im}}
\newcommand{\eq} [1] {\begin{equation}\label{#1}}
\newcommand{\en} {\end{equation}}
\newcommand{\la}{\lambda}
\newcommand{\BC}{{\mathbb C}}
\newcommand{\CC}[1]{{\mathbb C}^{#1\times #1}}
\newcommand{\BR}{{\mathbb R}}
\newcommand{\RR}[1]{{\mathbb R}^{#1\times #1}}
\newcommand{\BF}{{\mathbb F}}
\newcommand{\FF}[1]{{\mathbb F}^{#1\times #1}}
\newcommand{\BN}{{\mathbb N}}
\newcommand{\BZ}{{\mathbb Z}}
\newcommand{\BQ}{{\mathbb Q}}

\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\nn}{\nonumber}
\newcommand{\matl}{\left[ \begin{array}}
\newcommand{\matr}{\end{array} \right]}
\newcommand{\matls}{\left[ \begin{smallmatrix}}
\newcommand{\matrs}{\end{smallmatrix} \right]}
\newcommand{\isdef}{\stackrel{\triangle}{=}}
\newcommand{\pr}[1]{{#1}^{\prime}}
\newcommand{\inv}{^{-1}}
\newcommand{\row}[1]{{\rm row}_{#1}}
\newcommand{\col}[1]{{\rm col}_{#1}}
\newcommand{\arrowup}[1]{\stackrel{#1}{\SLeftarrow}}
\newcommand{\smin}{\stackrel{\min}{\sim}}
\newcommand{\jw}{\jmath \omega}
\newcommand{\omegan}{\omega_{\rm n}}
\newcommand{\omegad}{\omega_{\rm d}}
\newcommand{\omegar}{\omega_{\rm r}}
\newcommand{\omegani}{\omega_{{\rm n}i}}
\newcommand{\omegans}[1]{\omega_{{\rm n}_{#1}}}
\newcommand{\MSig}{{\mit\Sigma}}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\HS}{\hat S}
\newcommand{\HI}{\hat I}
\newcommand{\rmThat}{{\hat{\rm T}}}
\newcommand{\isge}{\stackrel{?}{\ge}}

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}

   
\newcommand{\defeq}{\stackrel{\triangle}{=}}
\newcommand{\real}{\raisebox{-0.05ex}{\textsf{\textup{I\hspace{-.12em}{\raisebox{1.435ex}
   {\rule{.2em}{.115ex}}\hspace{-.22em}R}}}}}

\newcommand{\detl}{\left | \begin{array}}
\newcommand{\detr}{\end{array} \right |}

\newcommand{\norml}{\left | \left |}
\newcommand{\normr}{\right | \right |}

\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}

\newcommand{\dpder}[2]{\displaystyle\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\der}[2]{\mbox{$\frac{d{#1}}{d{#2}}$}}
\newcommand{\dder}[2]{\displaystyle{\frac{d{#1}}{d{#2}}}}
\newcommand{\pder}[2]{\mbox{$\frac{\partial {#1}}{\partial {#2}}$}}
\newcommand{\dt}{{\rm d}t}
\newcommand{\dx}{{\rm d}x}
\newcommand{\p}{\partial}
\newcommand{\pt}{\partial_t}
\newcommand{\ptt}{\partial^2_t}
\newcommand{\px}{\partial_x}
\newcommand{\pxx}{\partial^2_x}
\newcommand{\pp}{\partial{^2}}

\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\mathsf T}}
%\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}

\newcommand{\rma}{{\rm a}}
\newcommand{\rmb}{{\rm b}}
\newcommand{\rmc}{{\rm c}}
\newcommand{\rmd}{{\rm d}}
\newcommand{\rme}{{\rm e}}
\newcommand{\rmf}{{\rm f}}
\newcommand{\rmg}{{\rm g}}
\newcommand{\rmh}{{\rm h}}
\newcommand{\rmi}{{\rm i}}
\newcommand{\rmj}{{\rm j}}
\newcommand{\rmk}{{\rm k}}
\newcommand{\rml}{{\rm l}}
\newcommand{\rmm}{{\rm m}}
\newcommand{\rmn}{{\rm n}}
\newcommand{\rmo}{{\rm o}}
\newcommand{\rmp}{{\rm p}}
\newcommand{\rmq}{{\rm q}}
\newcommand{\rmr}{{\rm r}}
\newcommand{\rms}{{\rm s}}
\newcommand{\rmt}{{\rm t}}
\newcommand{\rmu}{{\rm u}}
\newcommand{\rmv}{{\rm v}}
\newcommand{\rmw}{{\rm w}}
\newcommand{\rmx}{{\rm x}}
\newcommand{\rmy}{{\rm y}}
\newcommand{\rmz}{{\rm z}}

%\newcommand{\BBA}{{\mathbb A}}
\newcommand{\BBB}{{\mathbb B}}
%\newcommand{\BBC}{{\mathbb C}}
\newcommand{\BBD}{{\mathbb D}}
\newcommand{\BBE}{{\mathbb E}}
\newcommand{\BBF}{{\mathbb F}}
\newcommand{\BBG}{{\mathbb G}}
\newcommand{\BBH}{{\mathbb H}}
\newcommand{\BBI}{{\mathbb I}}
\newcommand{\BBJ}{{\mathbb J}}
\newcommand{\BBK}{{\mathbb K}}
\newcommand{\BBL}{{\mathbb L}}
\newcommand{\BBM}{{\mathbb M}}
%\newcommand{\BBN}{{\mathbb N}}
\newcommand{\BBO}{{\mathbb O}}
\newcommand{\BBP}{{\mathbb P}}
\newcommand{\BBQ}{{\mathbb Q}}
\newcommand{\BBR}{{\mathbb R}}
\newcommand{\BBS}{{\mathbb S}}
\newcommand{\BBT}{{\mathbb T}}
\newcommand{\BBU}{{\mathbb U}}
\newcommand{\BBV}{{\mathbb V}}
\newcommand{\BBW}{{\mathbb W}}
\newcommand{\BBX}{{\mathbb X}}
\newcommand{\BBY}{{\mathbb Y}}
\newcommand{\BBZ}{{\mathbb Z}}

\newcommand{\SA}{{\mathcal A}}
\newcommand{\SB}{{\mathcal B}}
\newcommand{\SC}{{\mathcal C}}
\newcommand{\SD}{{\mathcal D}}
\newcommand{\SE}{{\mathcal E}}
\newcommand{\SF}{{\mathcal F}}
\newcommand{\SG}{{\mathcal G}}
\newcommand{\SH}{{\mathcal H}}
%\newcommand{\SI}{{\mathcal I}}
\newcommand{\SJ}{{\mathcal J}}
\newcommand{\SK}{{\mathcal K}}
\newcommand{\SL}{{\mathcal L}}
\newcommand{\SM}{{\mathcal M}}
\newcommand{\SN}{{\mathcal N}}
\newcommand{\SO}{{\mathcal O}}
\newcommand{\SP}{{\mathcal P}}
\newcommand{\SQ}{{\mathcal Q}}
\newcommand{\SR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\ST}{{\mathcal T}}
\newcommand{\SU}{{\mathcal U}}
\newcommand{\SV}{{\mathcal V}}
\newcommand{\SW}{{\mathcal W}}
\newcommand{\SX}{{\mathcal X}}
\newcommand{\SY}{{\mathcal Y}}
\newcommand{\SZ}{{\mathcal Z}}

\newcommand{\BFA}{{\bf A}}
\newcommand{\BFB}{{\bf B}}
\newcommand{\BFC}{{\bf C}}
\newcommand{\BFD}{{\bf D}}
\newcommand{\BFE}{{\bf E}}
\newcommand{\BFF}{{\bf F}}
\newcommand{\BFG}{{\bf G}}
\newcommand{\BFH}{{\bf H}}
\newcommand{\BFI}{{\bf I}}
\newcommand{\BFJ}{{\bf J}}
\newcommand{\BFK}{{\bf K}}
\newcommand{\BFL}{{\bf L}}
\newcommand{\BFM}{{\bf M}}
\newcommand{\BFN}{{\bf N}}
\newcommand{\BFO}{{\bf O}}
\newcommand{\BFP}{{\bf P}}
\newcommand{\BFQ}{{\bf Q}}
\newcommand{\BFR}{{\bf R}}
\newcommand{\BFS}{{\bf S}}
\newcommand{\BFT}{{\bf T}}
\newcommand{\BFU}{{\bf U}}
\newcommand{\BFV}{{\bf V}}
\newcommand{\BFW}{{\bf W}}
\newcommand{\BFX}{{\bf X}}
\newcommand{\BFY}{{\bf Y}}
\newcommand{\BFZ}{{\bf Z}}





\newcommand{\bfa}{{\bf a}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfc}{{\bf c}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfe}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfg}{{\bf g}}
\newcommand{\bfh}{{\bf h}}
\newcommand{\bfi}{{\bf i}}
\newcommand{\bfj}{{\bf j}}
\newcommand{\bfk}{{\bf k}}
\newcommand{\bfl}{{\bf l}}
\newcommand{\bfm}{{\bf m}}
\newcommand{\bfn}{{\bf n}}
\newcommand{\bfo}{{\bf o}}
\newcommand{\bfp}{{\bf p}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfr}{{\bf r}}
\newcommand{\bfs}{{\bf s}}
\newcommand{\bft}{{\bf t}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfz}{{\bf z}}

==> TikzStuff.tex <==

\usepackage{tikz}
\usetikzlibrary{calc,patterns,decorations.pathmorphing,decorations.markings}
\usetikzlibrary{shapes,arrows}
\usepackage{verbatim}

\tikzstyle{block} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\usetikzlibrary{positioning}
\usetikzlibrary{math} 



\usepackage{tikz}
\usetikzlibrary{shapes,arrows,calc,positioning}
\tikzstyle{bigblock} = [draw, fill=blue!20, rectangle, 
    minimum height=6em, minimum width=8em]
\tikzstyle{medblock} = [draw, fill=blue!20, rectangle, 
    minimum height=4em, minimum width=4em]    
\tikzstyle{mux} = [draw, fill=black!20, rectangle, 
    minimum height=5em, minimum width=0.1em]    
\tikzstyle{smallblock} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=4em]
\tikzstyle{sum} = [draw, fill=blue!20, circle, node distance=1cm]
\tikzstyle{signal} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\tikzstyle{block} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=6em]
\tikzstyle{blockS} = [draw, fill=blue!20, rectangle, 
    minimum height=3em, minimum width=4em]    
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\usetikzlibrary{matrix}

\tikzset{add/.style n args={4}{
    minimum width=1mm,
    path picture={
        \draw[black, thick] 
            (path picture bounding box.south east) -- (path picture bounding box.north west)
            (path picture bounding box.south west) -- (path picture bounding box.north east);
        }
    }
}

\tikzset{Frame_into/.pic={
        code={\tikzset{scale=1}
        \tikzmath
            {
                \l  = 1;
                \Rc = 0.15;
            } 
        \draw [thick,->] (0, 0) -- +(\l, 0);
        \draw [thick,->] (0, 0) -- +(0, \l);
        % \node[circle, fill=white,black, minimum size=3pt] (circ) at (0,0) {} ; 
        % \draw [thick, black, fill=white] (0,0) circle [radius=.05];
        \draw [thick, fill=white] 
			    (0,0) circle [radius=\Rc];
	    \draw [thick] ({\Rc*cos(45)}, {0\Rc*sin(45)}) 
	               -- ({\Rc*cos(225)}, {0\Rc*sin(225)});
        \draw [thick] ({\Rc*cos(135)}, {0\Rc*sin(135)}) 
	               -- ({\Rc*cos(315)}, {0\Rc*sin(315)});
  }}
}

\tikzset{Frame_outof/.pic={
        code={\tikzset{scale=1}
        \tikzmath
            {
                \l  = 1;
                \Rc = 0.15;
            } 
        \draw [thick,->] (0, 0) -- +(\l, 0);
        \draw [thick,->] (0, 0) -- +(0, \l);
        % \node[circle, fill=white,black, minimum size=3pt] (circ) at (0,0) {} ; 
        % \draw [thick, black, fill=white] (0,0) circle [radius=.05];
        \draw [thick, fill=white] 
			    (0,0) circle [radius=\Rc];
	    \draw [thick, fill=black] 
			    (0,0) circle [radius={0.2*\Rc}];
  }}
}


\def\camera#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [fill=black](0,0) -- (2,2.5) -- (-2,2.5) -- cycle;
    \draw [fill=white,ultra thick](0,0) circle (1);
\end{scope}
}

\def\Frame#1#2{
\begin{scope}[shift={#1}, rotate=#2]
    \draw [thick,->] (0, 0) -- node[xshift=22, yshift=-10] {$\hat \jmath _\rmA$}  +(1, 0);
	\draw [thick,->] (0, 0) -- node[xshift=-10, yshift=-22] {$\hat k_\rmA$} +(0, 1);		
 	\node[draw,circle, fill=white, add={1}{2}{3}{4}] at (0,0) {} ; 
    % \draw [fill=black](0,0) -- (2,2.5) -- (-2,2.5) -- cycle;
    % \draw [fill=white,ultra thick](0,0) circle (1);
\end{scope}
}



% \makeatletter

% \pgfdeclareshape{record}{
% \inheritsavedanchors[from={rectangle}]
% \inheritbackgroundpath[from={rectangle}]
% \inheritanchorborder[from={rectangle}]
% \foreach \x in {center,north east,north west,north,south,south east,south west}{
% \inheritanchor[from={rectangle}]{\x}
% }
% \foregroundpath{
% \pgfpointdiff{\northeast}{\southwest}
% \pgf@xa=\pgf@x \pgf@ya=\pgf@y
% \northeast
% \pgfpathmoveto{\pgfpoint{0}{0.33\pgf@ya}}
% \pgfpathlineto{\pgfpoint{0}{-0.33\pgf@ya}}
% \pgfpathmoveto{\pgfpoint{0.33\pgf@xa}{0}}
% \pgfpathlineto{\pgfpoint{-0.33\pgf@xa}{0}}
% \pgfpathmoveto{\pgfpointadd{\southwest}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
% \pgfpathlineto{\pgfpointadd{\southwest}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
% \pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.5\pgf@xa}{-0.6\pgf@ya}}}
% \pgfpathlineto{\pgfpointadd{\northeast}{\pgfpoint{-0.33\pgf@xa}{-0.6\pgf@ya}}}
% }
% }
% \makeatother



==> discussions.tex <==
Extremum seeking control (ESC) constitutes a powerful technique for online optimization with theoretical guarantees for convergence to the neighborhood of the optimizer under well-understood conditions. However, ESC requires a nonconstant perturbation signal to provide persistent excitation to the target system to yield convergent results, which usually results in steady state oscillations. While certain techniques have been proposed to eliminate perturbations once the neighborhood of the minimizer is reached, system modifications and environmental perturbations can suddenly change the minimizer and nonconstant perturbations would once more be required to convergence to the new minimizer. Hence, this paper develops a retrospective cost-based ESC (RC/ESC) technique for online output minimization with a vanishing perturbation, that is, a perturbation that becomes zero as time increases independently from the state of the controller or the controlled system. The performance of the proposed algorithm is illustrated via numerical examples.
